BUMP: A Benchmark of Unfaithful Minimal Pairs for Meta-Evaluation of Faithfulness Metrics

The proliferation of automatic faithfulness metrics for summarization has produced a need for benchmarks to evaluate them. While existing benchmarks measure the correlation with human judgements of faithfulness on model-generated summaries, they are insufficient for diagnosing whether metrics are: 1) consistent, i.e., indicate lower faithfulness as errors are introduced into a summary, 2) effective on human-written texts, and 3) sensitive to different error types (as summaries can contain multiple errors). To address these needs, we present a benchmark of unfaithful minimal pairs (BUMP), a dataset of 889 human-written, minimally different summary pairs, where a single error is introduced to a summary from the CNN/DailyMail dataset to produce an unfaithful summary. We find BUMP complements existing benchmarks in a number of ways: 1) the summaries in BUMP are harder to discriminate and less probable under SOTA summarization models, 2) unlike non-pair-based datasets, BUMP can be used to measure the consistency of metrics, and reveals that the most discriminative metrics tend not to be the most consistent, and 3) unlike datasets containing generated summaries with multiple errors, BUMP enables the measurement of metrics' performance on individual error types.

==> backup.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{llcc}
        \toprule
        \midrule
                        &           & Task~1 & Task~2 \\
         \midrule
         \midrule
         Predicate      & Intrinsic & 99    & 17 \\
                        & Extrinsic & 99    & 28 \\
         Entity         & Intrinsic & 99    & 28 \\
                        & Extrinsic & 99    & 62 \\
         Circumstance   & Intrinsic & 99    & 22 \\
                        & Extrinsic & 99    & 33 \\
         Coreference    & -         & 99    & 1  \\
         Other          & -         & -     & 5  \\
         \midrule
         Total          &           & 693   & 196 \\
         \midrule
         \bottomrule
    \end{tabular}
    \caption{\dataset Dataset Statistics.}
    \label{tab:dataset-stats}
\end{table}


==> sections/30-Metrics.tex <==
\section{Faithfulness Evaluation Metrics}
{\clr[Shuyang]: some details on the metrics that are used in the paper, and how some of them are adapted to show the score between 0 and 1. Since we only have 4 pages, we should try to control the length of this section.}
{\clr[Rob]: I don't think this needs to be a long bullet pointed list. Makes more sense as a paragraph in Section 5, that lists the method names, and otherwise only lists information that is specific to our setup. }

\begin{itemize}
    \item \textsc{QuestEval}~\citep{scialom-etal-2021-questeval} is a QA-based metric that answers questions created from the summary using the document and vice versa. To obtain the evaluation score, the word overlaps between the answers given by the pre-trained QA model and the ground-truth answers used for generating the questions are aggregated over all questions.
    \item \textsc{SummaC}~\citep{laban-etal-2022-summac} is an entailment-based metric that first computes the entailment score between each pair of document and summary sentences. For each summary sentence, its entailment scores with document sentences are then binned into a histogram and transformed into the sentence-level faithfulness score via a 1-D convolutional layer. The mean of the sentence-level scores is then taken as the evaluation score.
    \item \textsc{CoCo}~\citep{xie-etal-2021-factual-consistency} is a model causality-based metric. We use its best-performing variant that masks document sentences that contain words in the summary. The difference between summary output probabilities given by a trained summarizer using the original document and the masked document is taken as the evaluation score. 
    \item \textsc{FactCC}
    \item \textsc{DAE}
    \item \textsc{$Q^2$}
    \item \textsc{QAFactEval}~\citep{fabbri-etal-2022-qafacteval} something better to have; should be easy to generate scores
    \item \textsc{BARTScore}~\citep{NEURIPS2021_e4d2b6e6} use the BART \citep{lewis-etal-2020-bart} model fine-tuned on CNNDM \citep{nallapati-etal-2016-abstractive}  which show the best performance to evaluate factualness, as shown in paper 
    \item \textsc{BERTScore}~\citep{bert-score} we follow the work in \cite{honovich-etal-2022-true} and use $deberta-xlarge$ \cite{he2020deberta}
    \item
    \textsc{BLEURT}
    \item \textsc{ROUGE} We use SacreROUGE\footnote{https://github.com/danieldeutsch/sacrerouge}~\citep{deutsch-roth-2020-sacrerouge} and specifically ROUGE-2 Precision
    \item \textsc{BLEU} we use SacreBLEU\footnote{https://github.com/mjpost/sacrebleu}~\citep{post-2018-call}
\end{itemize}
